Demystifying Oversmoothing in Attention-Based Graph Neural Networks

Oversmoothing in Graph Neural Networks (GNNs) refers to the phenomenon where increasing network depth leads to homogeneous node representations. While previous work has established that Graph Convolutional Networks (GCNs) exponentially lose expressive power, it remains controversial whether the graph attention mechanism can mitigate oversmoothing. In this work, we provide a definitive answer to this question through a rigorous mathematical analysis, by viewing attention-based GNNs as nonlinear time-varying dynamical systems and incorporating tools and techniques from the theory of products of inhomogeneous matrices and the joint spectral radius. We establish that, contrary to popular belief, the graph attention mechanism cannot prevent oversmoothing and loses expressive power exponentially. The proposed framework extends the existing results on oversmoothing for symmetric GCNs to a significantly broader class of GNN models, including random walk GCNs, Graph Attention Networks (GATs) and (graph) transformers. In particular, our analysis accounts for asymmetric, state-dependent and time-varying aggregation operators and a wide range of common nonlinear activation functions, such as ReLU, LeakyReLU, GELU and SiLU.

==> reference_app.tex <==
@book{Levin2008MarkovCA,
  title={Markov Chains and Mixing Times},
  author={David A. Levin and Yuval Peres and Elizabeth L. Wilmer},
  year={2008}
}

@book{Lax2002FA,
  title={Functional Analysis},
  author={Peter D. Lax},
  year={2002}
}

@inproceedings{Fey/Lenssen/2019,
  title={Fast Graph Representation Learning with {PyTorch Geometric}},
  author={Fey, Matthias and Lenssen, Jan E.},
  booktitle={ICLR Workshop on Representation Learning on Graphs and Manifolds},
  year={2019},
}

@inproceedings{Paszke2019PyTorchAI,
  title={PyTorch: An Imperative Style, High-Performance Deep Learning Library},
  author={Adam Paszke and Sam Gross and Francisco Massa and Adam Lerer and James Bradbury and Gregory Chanan and Trevor Killeen and Zeming Lin and Natalia Gimelshein and Luca Antiga and Alban Desmaison and Andreas K{\"o}pf and Edward Yang and Zach DeVito and Martin Raison and Alykhan Tejani and Sasank Chilamkurthy and Benoit Steiner and Lu Fang and Junjie Bai and Soumith Chintala},
  booktitle={NeurIPS},
  year={2019}
}

@inproceedings{Velickovic2017GraphAN,
  title={Graph Attention Networks},
  author={Petar Veli\v{c}kovi\'{c} and Guillem Cucurull and Arantxa Casanova and Adriana Romero and Pietro Li\`{o} and Yoshua Bengio},
  booktitle={ICLR},
  year={2018}
}

@article{theys2005joint,
  title={Joint Spectral Radius: theory and approximations},
  author={Theys, Jacques},
  journal={Ph. D. dissertation},
  year={2005},
}
